Influencing Competition Through Shelf Design

Shelf design decisions strongly influence product demand. In particular, placing products in desirable locations increases demand. This primary effect on shelf position is clear, but there is a secondary effect based on the relative positioning of nearby products. Intuitively, products located next to each other are more likely to be compared having positive and negative effects. On the one hand, locations closer to relatively strong products will be undesirable, as these strong products will draw demand from others -- an effect that is stronger for those in close proximity. On the other hand, because strong products tend to attract more traffic, locations closer to them elicit high consumer attention by increased visibility. Modifying the GEV class of models to allow demand to be moderated by competitors' proximity, these two effects emerge naturally. We found that although the competition effect is usually stronger, it is not always the dominating effect. Shelf displays can achieve higher profits by exploiting the relative influence on competition from shelf design to shift demand to higher profitability products. In the paper towel category, we found profitability differences of up to 7\% and displays with 3\% higher gross profits over the best shelf design present in our data.

==> Results_and_Tables/ptw_unused.tex <==
% table of data dimensions

\begin{table}[ht]
    \centering
\begin{tabular}{r|l}
    Number of products & 26 \\
    Number of stores & 44 \\
    Number of weeks (time frames) & 33
\end{tabular}
\end{table}



% listing of example data records

\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccc}
     & \multicolumn{3}{c}{Store 1,} & \multicolumn{3}{c}{Store 1,} & $\cdots$ & \multicolumn{3}{c}{Store 44,} \\
    Product & \multicolumn{3}{c}{Week 1} & \multicolumn{3}{c}{Week 2} & $\cdots$ & \multicolumn{3}{c}{Week 33} \\ \toprule
    $j$ & Moves & $\lambda_j$ & Price & Moves & $\lambda_j$ & Price & $\cdots$ & Moves & $\lambda_j$ & Price \\ \hline
1 & 102 & (65, 33) & 0.81 & 386 & (65, 33) & 0.75 & $\cdots$ & 7 & (90, 10) & 0.83\\ 
2 & 45 & (15, 33) & 0.69 & 36 & (15, 33) & 0.69 & $\cdots$ & 63 & (147, 10) & 0.69\\ 
3 & 160 & (175, 58) & 0.69 & 143 & (175, 58) & 0.69 & $\cdots$ & 60 & (170, 10) & 0.69\\ 
4 & 67 & (75, 58) & 0.93 & 49 & (75, 58) & 0.93 & $\cdots$ & 598 & (25, 58) & 0.69\\ 
5 & 67 & (100, 10) & 0.93 & 48 & (100, 10) & 0.93 & $\cdots$ & 585 & (60, 58) & 0.69\\ 
6 & --- & --- & --- & --- & --- & --- & $\cdots$ & 45 & (215, 58) & 1.55\\ 
7 & --- & --- & --- & --- & --- & --- & $\cdots$ & 40 & (190, 58) & 1.55\\ 
8 & 46 & (225, 58) & 2.79 & 27 & (225, 58) & 2.79 & $\cdots$ & 52 & (255, 58) & 2.94\\ 
9 & 135 & (140, 10) & 0.59 & 81 & (140, 10) & 0.59 & $\cdots$ & 209 & (120, 10) & 0.69\\ 
10 & 3 & (275, 58) & 0.96 & --- & --- & --- & $\cdots$ & --- & --- & ---\\ 
     $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & $\vdots$ & & $\vdots$ & $\vdots$ & $\vdots$
     \end{tabular}
    }
    \caption{Sample data for the first 10 out of $26$ products. Some products were not on display at some stores in some weeks and we indicated this by `---'. Although omitted in this table, the profit data is also available for each store and week.}
    \label{table:sampledata}
\end{table}

==> Results_and_Tables/resultptw_pos.tex <==

\begin{table}[H]
\begin{tabular}{lccccc}
    \toprule
                   & \textbf{RMSE}      & \textbf{RMSE}       &                   &                 & \textbf{Price} \\
     \textbf{Model}& \textbf{In-Sample} & \textbf{Out-Sample} & \textbf{$\gamma^*$} & \textbf{$\rho$} & \textbf{sensitivity} \\
    \hline
\multirow{2}{*}{$MNL$} & \multirow{2}{*}{\color[rgb]{1.0,0.0,0} 2.09\%} & \multirow{2}{*}{\color[rgb]{1.0,0.0,0} 1.78\%} & --- & --- & 3.32\\ 
 & &  & --- & --- & (0.01)\\ 
\multirow{2}{*}{$MNL$ w/A} & \multirow{2}{*}{\color[rgb]{0.5219818598716084,0.4780181401283916,0} 1.09\%} & \multirow{2}{*}{\color[rgb]{0.9910854255780633,0.00891457442193666,0} 1.76\%} & --- & --- & 3.44\\ 
 & &  & --- & --- & (0.02)\\ 
\multirow{2}{*}{$NESTED$ w/A} & \multirow{2}{*}{\color[rgb]{0.5224835190143754,0.4775164809856246,0} 1.09\%} & \multirow{2}{*}{\color[rgb]{0.9501626028658127,0.04983739713418733,0} 1.69\%} & --- & 0.96 & 3.43\\ 
 & &  & --- & (0.00) & (0.02)\\ 
\multirow{2}{*}{$NESTED$} & \multirow{2}{*}{\color[rgb]{0.9338472517975642,0.06615274820243577,0} 1.95\%} & \multirow{2}{*}{\color[rgb]{0.9101921291035487,0.08980787089645126,0} 1.62\%} & --- & 0.89 & 3.32\\ 
 & &  & --- & (0.01) & (0.02)\\ 
\multirow{2}{*}{$NCL^{exp}$ w/A} & \multirow{2}{*}{\color[rgb]{0.04603912189325343,0.9539608781067466,0} 0.10\%} & \multirow{2}{*}{\color[rgb]{0.3545141995548909,0.6454858004451092,0} 0.63\%} & 0.27 & 0.25 & 2.73\\ 
 & &  & (0.22) & (0.01) & (0.06)\\ 
\multirow{2}{*}{$NCL^{inv}$ w/A} & \multirow{2}{*}{\color[rgb]{0.07724998112417727,0.9227500188758228,0} 0.16\%} & \multirow{2}{*}{\color[rgb]{0.3520520411486506,0.6479479588513495,0} 0.62\%} & 10.44 & 0.25 & 2.74\\ 
 & &  & (5.18) & (0.01) & (0.02)\\ 
\multirow{2}{*}{$NCL^{exp}$} & \multirow{2}{*}{\color[rgb]{0.29772606408594,0.70227393591406,0} 0.62\%} & \multirow{2}{*}{\color[rgb]{0.10464281713797492,0.895357182862025,0} 0.19\%} & 0.01 & 0.25 & 2.73\\ 
 & &  & (0.01) & (0.11) & (0.10)\\ 
\multirow{2}{*}{$NCL^{inv}$} & \multirow{2}{*}{\color[rgb]{0.30121695112498414,0.6987830488750159,0} 0.63\%} & \multirow{2}{*}{\color[rgb]{0.10965694539968361,0.8903430546003164,0} 0.19\%} & 0.00 & 0.25 & 2.73\\ 
 & &  & (0.00) & (0.01) & (0.02)\\ 
\multirow{2}{*}{$NCL^{exp}$ w/A \& Pos} & \multirow{2}{*}{\color[rgb]{0.0,1.0,0} 0.00\%} & \multirow{2}{*}{\color[rgb]{0.2217516258514727,0.7782483741485273,0} 0.39\%} & 0.28 & 0.30 & 2.74\\ 
 & &  & (0.18) & (0.03) & (0.05)\\ 
\multirow{2}{*}{$NCL^{inv}$ w/A \& Pos} & \multirow{2}{*}{\color[rgb]{0.025590162213433063,0.974409837786567,0} 0.05\%} & \multirow{2}{*}{\color[rgb]{0.2013471882082858,0.7986528117917142,0} 0.36\%} & 11.54 & 0.30 & 2.74\\ 
 & &  & (5.81) & (0.01) & (0.02)\\ 
\multirow{2}{*}{$NCL^{exp}$ \& Pos} & \multirow{2}{*}{\color[rgb]{0.25488274139687367,0.7451172586031263,0} 0.53\%} & \multirow{2}{*}{\color[rgb]{0.0,1.0,0} 0.00\%} & 0.01 & 0.30 & 2.73\\ 
 & &  & (0.01) & (0.07) & (0.05)\\ 
\multirow{2}{*}{$NCL^{inv}$ \& Pos} & \multirow{2}{*}{\color[rgb]{0.2570325125059871,0.7429674874940129,0} 0.54\%} & \multirow{2}{*}{\color[rgb]{0.004536093622148986,0.995463906377851,0} 0.01\%} & 0.00 & 0.30 & 2.73\\ 
 & &  & (0.00) & (0.01) & (0.01)\\  
\bottomrule 
\end{tabular}%} 
\caption{Estimation with Paper Towel (PTW) Category. Asterisks (*) indicate the values in the column are multiplied by 100 to ease the presentation.}
\label{tab:PTW}
\end{table} 


==> Results_and_Tables/resultptwblpR10.tex <==
%R = 10

\begin{table}[H]
\begin{tabular}{lccccc}
    \toprule
                   & \textbf{RMSE}      & \textbf{RMSE}       &                   &                 & \textbf{Price} \\
     \textbf{Model}& \textbf{In-Sample} & \textbf{Out-Sample} & \textbf{$\gamma$} & \textbf{$\rho$} & \textbf{sensitivity} \\
    \hline 
$MNL$ & \color[rgb]{1.0,0.0,0} 2.60\% & \color[rgb]{1.0,0.0,0} 3.23\% & & & 3.19\\ 
$MNL$ w/A & \color[rgb]{0.623445529270127,0.376554470729873,0} 1.62\% & \color[rgb]{0.7574517119144492,0.24254828808555084,0} 2.45\% & &  & 3.26\\ 
$NCL^{exp}$ w/A & \color[rgb]{0.0,1.0,0} 0.00\% & \color[rgb]{0.21823095864731712,0.7817690413526829,0} 0.70\% & 0.01 & 0.247 & 2.67\\ 
$NCL^{inv}$ w/A & \color[rgb]{0.049803004295600375,0.9501969957043996,0} 0.13\% & \color[rgb]{0.14117325154778904,0.858826748452211,0} 0.46\% & 0.13 & 0.249 & 2.71\\ 
$NCL^{exp}$ & \color[rgb]{0.2146289834804084,0.7853710165195916,0} 0.56\% & \color[rgb]{0.1547304670797116,0.8452695329202884,0} 0.50\% & 0.00 & 0.244 & 2.67\\ 
$NCL^{inv}$ & \color[rgb]{0.22770779550357215,0.7722922044964279,0} 0.59\% & \color[rgb]{0.18052614103301906,0.819473858966981,0} 0.58\% & 0.02 & 0.242 & 2.71\\ 
$NCL^{exp}$ w/A \& Pos & \color[rgb]{0.0589189401154016,0.9410810598845984,0} 0.15\% & \color[rgb]{0.3245917387984834,0.6754082612015166,0} 1.05\% & 0.02 & 0.297 & 2.72\\ 
$NCL^{inv}$ w/A \& Pos & \color[rgb]{0.09510936848433676,0.9048906315156633,0} 0.25\% & \color[rgb]{0.13296359883747147,0.8670364011625286,0} 0.43\% & 0.14 & 0.295 & 2.72\\ 
$NCL^{exp}$ \& Pos & \color[rgb]{0.30405906078299055,0.6959409392170095,0} 0.79\% & \color[rgb]{0.6542332601915494,0.34576673980845063,0} 2.11\% & 0.01 & 0.285 & 2.74\\ 
$NCL^{inv}$ \& Pos & \color[rgb]{0.011745149874781903,0.9882548501252181,0} 0.03\% & \color[rgb]{0.0,1.0,0} 0.00\% & 0.02 & 0.290 & 2.71\\ 
\bottomrule 
\end{tabular} 
\caption{Estimation of heterogeneous model with Paper Towel (PTW) Category}
\label{tab:PTW_BLP}
\end{table} 


==> Results_and_Tables/resultptwblp_pos.tex <==
% R = 30
\begin{table}[H]
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
    \toprule
                   & \textbf{RMSE}      & \textbf{RMSE}       &                   &                 & \textbf{Price} \\
     \textbf{Model}& \textbf{In-Sample} & \textbf{Out-Sample} & \textbf{$\gamma^*$} & \textbf{$\rho$} & \textbf{sensitivity} & $\Pi_0^*$ & $L_{0,0}^*$ \\
    \hline 
\multirow{2}{*}{$MNL$} & \multirow{2}{*}{\color[rgb]{1.0,0.0,0} 2.28\%} & \multirow{2}{*}{\color[rgb]{1.0,0.0,0} 2.77\%} & --- & --- & 3.12 & -6.19 & -10.20\\ 
 & &  & --- & --- & (0.00) & \small{(0.003)} & \small{(0.002)}\\ 
\multirow{2}{*}{$MNL$ w/A} & \multirow{2}{*}{\color[rgb]{0.6540344433129324,0.34596555668706763,0} 1.49\%} & \multirow{2}{*}{\color[rgb]{0.7425309086449727,0.25746909135502727,0} 2.06\%} & --- & --- & 3.22 & -7.61 & 8.83\\ 
 & &  & --- & --- & (0.00) & \small{(0.004)} & \small{(0.001)}\\ 
\multirow{2}{*}{$NESTED$ w/A} & \multirow{2}{*}{\color[rgb]{0.614338746025182,0.385661253974818,0} 1.40\%} & \multirow{2}{*}{\color[rgb]{0.6460793203429146,0.3539206796570854,0} 1.79\%} & --- & 0.96 & 3.22 & -7.22 & -2.38\\ 
 & &  & --- & (0.00) & (0.00) & \small{(0.002)} & \small{(0.000)}\\ 
\multirow{2}{*}{$NESTED$} & \multirow{2}{*}{\color[rgb]{0.9187353532728061,0.08126464672719391,0} 2.10\%} & \multirow{2}{*}{\color[rgb]{0.9354247526569579,0.0645752473430421,0} 2.60\%} & --- & 0.89 & 3.15 & -4.96 & 9.03\\ 
 & &  & --- & (0.00) & (0.00) & \small{(0.003)} & \small{(0.001)}\\ 
\multirow{2}{*}{$NCL^{exp}$ w/A} & \multirow{2}{*}{\color[rgb]{0.0011729408041854553,0.9988270591958145,0} 0.00\%} & \multirow{2}{*}{\color[rgb]{0.016329682402550765,0.9836703175974493,0} 0.05\%} & 0.26 & 0.25 & 2.70 & -0.68 & -2.78\\ 
 & &  & (0.05) & (0.00) & (0.00) & \small{(0.167)} & \small{(0.047)}\\ 
\multirow{2}{*}{$NCL^{inv}$ w/A} & \multirow{2}{*}{\color[rgb]{0.06185378553015753,0.9381462144698425,0} 0.14\%} & \multirow{2}{*}{\color[rgb]{0.049221391872559576,0.9507786081274404,0} 0.14\%} & 12.55 & 0.25 & 2.72 & -0.38 & -2.94\\ 
 & &  & (0.04) & (0.00) & (0.00) & \small{(0.055)} & \small{(0.030)}\\ 
\multirow{2}{*}{$NCL^{exp}$} & \multirow{2}{*}{\color[rgb]{0.24770673041912605,0.752293269580874,0} 0.56\%} & \multirow{2}{*}{\color[rgb]{0.165485932544984,0.834514067455016,0} 0.46\%} & 0.05 & 0.24 & 2.70 & -0.63 & -3.05\\ 
 & &  & (0.06) & (0.00) & (0.00) & \small{(0.166)} & \small{(0.043)}\\ 
\multirow{2}{*}{$NCL^{inv}$} & \multirow{2}{*}{\color[rgb]{0.24699188082810244,0.7530081191718976,0} 0.56\%} & \multirow{2}{*}{\color[rgb]{0.16490927774825,0.83509072225175,0} 0.46\%} & 1.84 & 0.24 & 2.71 & -0.14 & 3.23\\ 
 & &  & (0.02) & (0.00) & (0.00) & \small{(0.043)} & \small{(0.019)}\\ 
\multirow{2}{*}{$NCL^{exp}$ w/A \& Pos} & \multirow{2}{*}{\color[rgb]{0.0,1.0,0} 0.00\%} & \multirow{2}{*}{\color[rgb]{0.03597237734952754,0.9640276226504725,0} 0.10\%} & 0.54 & 0.30 & 2.71 & -0.24 & -3.20\\ 
 & &  & (0.01) & (0.00) & (0.00) & \small{(0.048)} & \small{(0.012)}\\ 
\multirow{2}{*}{$NCL^{inv}$ w/A \& Pos} & \multirow{2}{*}{\color[rgb]{0.037947889859094176,0.9620521101409059,0} 0.09\%} & \multirow{2}{*}{\color[rgb]{0.0,1.0,0} 0.00\%} & 13.95 & 0.30 & 2.72 & -0.27 & -3.31\\ 
 & &  & (0.07) & (0.00) & (0.00) & \small{(0.023)} & \small{(0.013)}\\ 
\multirow{2}{*}{$NCL^{exp}$ \& Pos} & \multirow{2}{*}{\color[rgb]{0.23652553647106267,0.7634744635289373,0} 0.54\%} & \multirow{2}{*}{\color[rgb]{0.14994249651375804,0.850057503486242,0} 0.42\%} & 0.29 & 0.29 & 2.69 & -0.77 & -3.04\\ 
 & &  & (0.67) & (0.00) & (0.01) & \small{(0.733)} & \small{(0.330)}\\ 
\multirow{2}{*}{$NCL^{inv}$ \& Pos} & \multirow{2}{*}{\color[rgb]{0.1750857778216256,0.8249142221783744,0} 0.40\%} & \multirow{2}{*}{\color[rgb]{0.10109541980143602,0.898904580198564,0} 0.28\%} & 1.83 & 0.29 & 2.71 & -0.02 & -3.35\\ 
 & &  & (0.03) & (0.00) & (0.00) & \small{(0.015)} & \small{(0.007)}\\ 
\bottomrule 
\end{tabular} 
\caption{Estimation of heterogeneous model with Paper Towel (PTW) Category. Asterisks (*) indicate the values in the column are multiplied by 100 to ease the presentation.}
\label{tab:PTW_BLP}
}
\end{table} 



==> Results_and_Tables/results_tti.tex <==
%Currently not using these results.  Will only report PTW in the paper, and leave TTI for an appendix.

\textbf{Bathroom Tissue (TTI):} We selected this category for similar reasons than PTW, however the experimental design aim to inhibit price competition by reorganizing products by number of rolls per pack instead of brand. In this experiment 2 treatments were included in addition to the control group.

\textbf{TTI control design:} The stores originally by brands and separate single-rolls from the multi-rolls as in Figure $\ref{fig:tti_control}$

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{graphics/TTI_control_design.JPG}
    \caption{\small{TTI Control design}}
    \label{fig:tti_control}
\end{figure}

\textbf{TTI Treatment 1 and 2 –Hard to compare 1–} organizing by number of rolls per package in two different versions, as shown in Figures $\ref{fig:tti_design1}$ and $\ref{fig:tti_design2}$ 

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{graphics/TTI_exp1_design.JPG}
    \caption{\small{TTI Shelf treatment 1.}}
    \label{fig:tti_design1}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{graphics/TTI_exp2_design.JPG}
    \caption{\small{TTI Shelf treatment 2.}}
    \label{fig:tti_design2}
\end{figure}

\input{resultttish}

==> Results_and_Tables/resultttish.tex <==
\begin{table}[H]
\begin{tabular}{lccccc}
    \toprule
                  & \textbf{RMSE}      & \textbf{RMSE}       &                   &                 & \textbf{Price} \\
    \textbf{Model}& \textbf{In-Sample} & \textbf{Out-Sample} & \textbf{$\gamma$} & \textbf{$\rho$} & \textbf{sensitivity} \\
    \hline
\multirow{2}{*}{$MNL$} & \multirow{2}{*}{\color[rgb]{1.0,0.0,0} 2.12\%} & \multirow{2}{*}{\color[rgb]{1.0,0.0,0} 8.21\%} & --- & --- & 6.91\\ 
 & &  & --- & --- & (0.02)\\ 
\multirow{2}{*}{$MNL$ w/A} & \multirow{2}{*}{\color[rgb]{0.24233239616643393,0.7576676038335661,0} 0.51\%} & \multirow{2}{*}{\color[rgb]{0.30130970756386366,0.6986902924361363,0} 2.47\%} & --- & --- & 7.13\\ 
 & &  & --- & --- & (0.02)\\ 
\multirow{2}{*}{$NESTED$ w/A} & \multirow{2}{*}{\color[rgb]{0.38702466826482396,0.612975331735176,0} 0.82\%} & \multirow{2}{*}{\color[rgb]{0.12357839534448797,0.876421604655512,0} 1.02\%} & --- & 0.86 & 6.80\\ 
 & &  & --- & (0.01) & (0.03)\\ 
\multirow{2}{*}{$NESTED$} & \multirow{2}{*}{\color[rgb]{0.8431237039434282,0.15687629605657183,0} 1.79\%} & \multirow{2}{*}{\color[rgb]{0.6025305490137725,0.39746945098622755,0} 4.95\%} & --- & 0.80 & 6.60\\ 
 & &  & --- & (0.01) & (0.03)\\ 
\multirow{2}{*}{$NCL^{exp}$ w/A} & \multirow{2}{*}{\color[rgb]{0.4074324161963161,0.5925675838036839,0} 0.86\%} & \multirow{2}{*}{\color[rgb]{0.0325339185097124,0.9674660814902876,0} 0.27\%} & 0.03 & 0.33 & 6.21\\ 
 & &  & (0.00) & (0.05) & (0.04)\\ 
\multirow{2}{*}{$NCL^{inv}$ w/A} & \multirow{2}{*}{\color[rgb]{0.0,1.0,0} 0.00\%} & \multirow{2}{*}{\color[rgb]{0.0,1.0,0} 0.00\%} & 1.51 & 0.41 & 6.35\\ 
 & &  & (0.03) & (0.01) & (0.03)\\ 
\multirow{2}{*}{$NCL^{exp}$} & \multirow{2}{*}{\color[rgb]{0.5987689205565698,0.40123107944343017,0} 1.27\%} & \multirow{2}{*}{\color[rgb]{0.48665572582550454,0.5133442741744955,0} 4.00\%} & 0.04 & 0.39 & 6.24\\ 
 & &  & (0.01) & (0.01) & (0.04)\\ 
\multirow{2}{*}{$NCL^{inv}$} & \multirow{2}{*}{\color[rgb]{0.6622896220271676,0.33771037797283243,0} 1.40\%} & \multirow{2}{*}{\color[rgb]{0.5248803371240761,0.4751196628759239,0} 4.31\%} & 1.75 & 0.42 & 6.23\\ 
 & &  & (0.05) & (0.03) & (0.05)\\ 
\multirow{2}{*}{$NCL^{exp}$ w/A \& Pos} & \multirow{2}{*}{\color[rgb]{0.21056251030305412,0.7894374896969458,0} 0.45\%} & \multirow{2}{*}{\color[rgb]{0.11442734294104359,0.8855726570589564,0} 0.94\%} & 0.06 & 0.57 & 6.48\\ 
 & &  & (0.01) & (0.03) & (0.03)\\ 
\multirow{2}{*}{$NCL^{inv}$ w/A \& Pos} & \multirow{2}{*}{\color[rgb]{0.09823596291304774,0.9017640370869523,0} 0.21\%} & \multirow{2}{*}{\color[rgb]{0.22558344917554735,0.7744165508244527,0} 1.85\%} & 9.26 & 0.65 & 6.67\\ 
 & &  & (0.03) & (0.01) & (0.02)\\ 
\multirow{2}{*}{$NCL^{exp}$ \& Pos} & \multirow{2}{*}{\color[rgb]{0.6366931613031105,0.3633068386968895,0} 1.35\%} & \multirow{2}{*}{\color[rgb]{0.6501777683490476,0.3498222316509524,0} 5.34\%} & 0.08 & 0.57 & 6.42\\ 
 & &  & (0.01) & (0.01) & (0.03)\\ 
\multirow{2}{*}{$NCL^{inv}$ \& Pos} & \multirow{2}{*}{\color[rgb]{0.6412387964449687,0.35876120355503127,0} 1.36\%} & \multirow{2}{*}{\color[rgb]{0.7924385632498107,0.20756143675018934,0} 6.51\%} & 6.15 & 0.63 & 6.52\\ 
 & &  & (0.26) & (0.01) & (0.03)\\ 
\bottomrule 
\end{tabular}%} 
\caption{Estimation with Toilet Tissue (TTI) Category}
\label{tab:TTI}
\end{table} 


==> Results_and_Tables/table_shelfdesign_a.tex <==
\begin{table}[H]
    \caption{Values of $f^{inv}_{jj'}$ for shelf Design 1 and Design 2 in Figure \ref{fig:D1D2}.}
    \label{tab:example_proximity}
    \begin{subtable}{.5\linewidth}
      \centering
        \caption{Design 1}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{cc|ccccc}
        \multicolumn{2}{c|}{\multirow{2}{*}{$f^{inv}_{jj'}$}} & \multicolumn{5}{c}{$j'$} \\
        & & 1 & 2 & 3 & 4 & 5 \\
        \toprule
        \multirow{5}{*}{$j$} 
 & 1 & 0.000 & 0.167 & 0.077 & 0.124 & 0.064\\
 & 2 & 0.167 & 0.000 & 0.143 & 0.137 & 0.094\\
 & 3 & 0.077 & 0.143 & 0.000 & 0.088 & 0.141\\
 & 4 & 0.124 & 0.137 & 0.088 & 0.000 & 0.100\\
 & 5 & 0.064 & 0.094 & 0.141 & 0.100 & 0.000\\
        \bottomrule
    \end{tabular}}
    \end{subtable}
   \begin{subtable}{.5\linewidth}
      \centering
        \caption{Design 2}
    \resizebox{0.8\textwidth}{!}{\begin{tabular}{cc|ccccc}
        \multicolumn{2}{c|}{\multirow{2}{*}{$f^{inv}_{jj'}$}} & \multicolumn{5}{c}{$j'$} \\
        & & 1 & 2 & 3 & 4 & 5 \\
        \toprule
        \multirow{5}{*}{$j$} 
 & 1 & 0.000 & 0.116 & 0.125 & 0.116 & 0.167\\
 & 2 & 0.116 & 0.000 & 0.068 & 0.100 & 0.141\\
 & 3 & 0.125 & 0.068 & 0.000 & 0.131 & 0.071\\
 & 4 & 0.116 & 0.100 & 0.131 & 0.000 & 0.077\\
 & 5 & 0.167 & 0.141 & 0.071 & 0.077 & 0.000\\
        \bottomrule
    \end{tabular}}
    \end{subtable}
\end{table}

==> Results_and_Tables/table_shelfdesign_b.tex <==
\begin{table}[H]
    \caption{Values of $\alpha^{(\Lambda_k)}_{j,jj'}$ for shelf Design 1 and Design 2 in Figure \ref{fig:D1D2}. The superscript value in parentheses refers to the shelf design. Note that the sum of each row is 1.}
    \label{tab:example_allocation}
    \begin{subtable}{.5\linewidth}
      \centering
        \caption{Design 1}
\resizebox{0.8\textwidth}{!}{\begin{tabular}{cc|ccccc}
        \multicolumn{2}{c|}{\multirow{2}{*}{$\alpha^{(\Lambda_1)}_{j,jj'}$}} & \multicolumn{5}{c}{$j'$} \\
        & & 1 & 2 & 3 & 4 & 5 \\
        \toprule
        \multirow{5}{*}{$j$} 
 & 1 & 0.000 & 0.386 & 0.178 & 0.287 & 0.148\\
 & 2 & 0.308 & 0.000 & 0.264 & 0.254 & 0.174\\
 & 3 & 0.171 & 0.318 & 0.000 & 0.195 & 0.315\\
 & 4 & 0.276 & 0.306 & 0.195 & 0.000 & 0.223\\
 & 5 & 0.160 & 0.236 & 0.354 & 0.250 & 0.000\\
        \bottomrule
    \end{tabular}}
    \end{subtable}
   \begin{subtable}{.5\linewidth}
      \centering
        \caption{Design 2}
    \resizebox{0.8\textwidth}{!}{\begin{tabular}{cc|ccccc}
        \multicolumn{2}{c|}{\multirow{2}{*}{$\alpha^{(\Lambda_2)}_{j,jj'}$}} & \multicolumn{5}{c}{$j'$} \\
        & & 1 & 2 & 3 & 4 & 5 \\
        \toprule
        \multirow{5}{*}{$j$} 
 & 1 & 0.000 & 0.222 & 0.238 & 0.222 & 0.318\\
 & 2 & 0.273 & 0.000 & 0.159 & 0.235 & 0.332\\
 & 3 & 0.316 & 0.171 & 0.000 & 0.332 & 0.181\\
 & 4 & 0.274 & 0.236 & 0.310 & 0.000 & 0.181\\
 & 5 & 0.365 & 0.310 & 0.157 & 0.168 & 0.000\\
        \bottomrule
    \end{tabular}}
    \end{subtable}
\end{table}
